Joint Localization, Synchronization and Mapping via Phase-Coherent Distributed Arrays

Extremely large-scale antenna array (ELAA) systems emerge as a promising technology in beyond 5G and 6G wireless networks to support the deployment of distributed architectures. This paper explores the use of ELAAs to enable joint localization, synchronization and mapping in sub-6 GHz uplink channels, capitalizing on the near-field effects of phase-coherent distributed arrays. We focus on a scenario where a single-antenna user equipment (UE) communicates with a network of access points (APs) distributed in an indoor environment, considering both specular reflections from walls and scattering from objects. The UE is assumed to be unsynchronized to the network, while the APs can be time- and phase-synchronized to each other. We formulate the problem of joint estimation of location, clock offset and phase offset of the UE, and the locations of scattering points (SPs) (i.e., mapping). Through comprehensive Fisher information analysis, we assess the impact of bandwidth, AP array size, wall reflections, SPs and phase synchronization on localization accuracy. Furthermore, we derive the maximum-likelihood (ML) estimator, which optimally combines the information collected by all the distributed arrays. To overcome its intractable high dimensionality, we propose a novel three-step algorithm that first estimates phase offset leveraging carrier phase information of line-of-sight (LoS) paths, then determines the UE location and clock offset via LoS paths and wall reflections, and finally locates SPs using a null-space transformation technique. Simulation results demonstrate the effectiveness of our approach in distributed architectures supported by radio stripes (RSs) -- an innovative alternative for implementing ELAAs -- while revealing the benefits of carrier phase exploitation and showcasing the interplay between delay and angular information under different bandwidth regimes.

==> Figures/Estimator_figures/cost_coherent_20_dB_pos/cost_coherent_20_dB_pos.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=2.3735,
xmax=3.4,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={Y-Coordinate [m]},
ymin=2.5,
ymax=3.5297,
ylabel style={font=\color{white!15!black}},
ylabel={X-Coordinate [m]},
zmin=-10.1984660255774,
zmax=0,
zlabel style={font=\color{white!15!black}},
zlabel={ML Cost Function [dB]},
view={45}{19},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
zmajorgrids,
legend style={at={(0.61,0.264)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]

\addplot3[%
surf,
shader=flat corner, fill=white, z buffer=sort, colormap={mymap}{[1pt] rgb(0pt)=(0.2422,0.1504,0.6603); rgb(1pt)=(0.2444,0.1534,0.6728); rgb(2pt)=(0.2464,0.1569,0.6847); rgb(3pt)=(0.2484,0.1607,0.6961); rgb(4pt)=(0.2503,0.1648,0.7071); rgb(5pt)=(0.2522,0.1689,0.7179); rgb(6pt)=(0.254,0.1732,0.7286); rgb(7pt)=(0.2558,0.1773,0.7393); rgb(8pt)=(0.2576,0.1814,0.7501); rgb(9pt)=(0.2594,0.1854,0.761); rgb(11pt)=(0.2628,0.1932,0.7828); rgb(12pt)=(0.2645,0.1972,0.7937); rgb(13pt)=(0.2661,0.2011,0.8043); rgb(14pt)=(0.2676,0.2052,0.8148); rgb(15pt)=(0.2691,0.2094,0.8249); rgb(16pt)=(0.2704,0.2138,0.8346); rgb(17pt)=(0.2717,0.2184,0.8439); rgb(18pt)=(0.2729,0.2231,0.8528); rgb(19pt)=(0.274,0.228,0.8612); rgb(20pt)=(0.2749,0.233,0.8692); rgb(21pt)=(0.2758,0.2382,0.8767); rgb(22pt)=(0.2766,0.2435,0.884); rgb(23pt)=(0.2774,0.2489,0.8908); rgb(24pt)=(0.2781,0.2543,0.8973); rgb(25pt)=(0.2788,0.2598,0.9035); rgb(26pt)=(0.2794,0.2653,0.9094); rgb(27pt)=(0.2798,0.2708,0.915); rgb(28pt)=(0.2802,0.2764,0.9204); rgb(29pt)=(0.2806,0.2819,0.9255); rgb(30pt)=(0.2809,0.2875,0.9305); rgb(31pt)=(0.2811,0.293,0.9352); rgb(32pt)=(0.2813,0.2985,0.9397); rgb(33pt)=(0.2814,0.304,0.9441); rgb(34pt)=(0.2814,0.3095,0.9483); rgb(35pt)=(0.2813,0.315,0.9524); rgb(36pt)=(0.2811,0.3204,0.9563); rgb(37pt)=(0.2809,0.3259,0.96); rgb(38pt)=(0.2807,0.3313,0.9636); rgb(39pt)=(0.2803,0.3367,0.967); rgb(40pt)=(0.2798,0.3421,0.9702); rgb(41pt)=(0.2791,0.3475,0.9733); rgb(42pt)=(0.2784,0.3529,0.9763); rgb(43pt)=(0.2776,0.3583,0.9791); rgb(44pt)=(0.2766,0.3638,0.9817); rgb(45pt)=(0.2754,0.3693,0.984); rgb(46pt)=(0.2741,0.3748,0.9862); rgb(47pt)=(0.2726,0.3804,0.9881); rgb(48pt)=(0.271,0.386,0.9898); rgb(49pt)=(0.2691,0.3916,0.9912); rgb(50pt)=(0.267,0.3973,0.9924); rgb(51pt)=(0.2647,0.403,0.9935); rgb(52pt)=(0.2621,0.4088,0.9946); rgb(53pt)=(0.2591,0.4145,0.9955); rgb(54pt)=(0.2556,0.4203,0.9965); rgb(55pt)=(0.2517,0.4261,0.9974); rgb(56pt)=(0.2473,0.4319,0.9983); rgb(57pt)=(0.2424,0.4378,0.9991); rgb(58pt)=(0.2369,0.4437,0.9996); rgb(59pt)=(0.2311,0.4497,0.9995); rgb(60pt)=(0.225,0.4559,0.9985); rgb(61pt)=(0.2189,0.462,0.9968); rgb(62pt)=(0.2128,0.4682,0.9948); rgb(63pt)=(0.2066,0.4743,0.9926); rgb(64pt)=(0.2006,0.4803,0.9906); rgb(65pt)=(0.195,0.4861,0.9887); rgb(66pt)=(0.1903,0.4919,0.9867); rgb(67pt)=(0.1869,0.4975,0.9844); rgb(68pt)=(0.1847,0.503,0.9819); rgb(69pt)=(0.1831,0.5084,0.9793); rgb(70pt)=(0.1818,0.5138,0.9766); rgb(71pt)=(0.1806,0.5191,0.9738); rgb(72pt)=(0.1795,0.5244,0.9709); rgb(73pt)=(0.1785,0.5296,0.9677); rgb(74pt)=(0.1778,0.5349,0.9641); rgb(75pt)=(0.1773,0.5401,0.9602); rgb(76pt)=(0.1768,0.5452,0.956); rgb(77pt)=(0.1764,0.5504,0.9516); rgb(78pt)=(0.1755,0.5554,0.9473); rgb(79pt)=(0.174,0.5605,0.9432); rgb(80pt)=(0.1716,0.5655,0.9393); rgb(81pt)=(0.1686,0.5705,0.9357); rgb(82pt)=(0.1649,0.5755,0.9323); rgb(83pt)=(0.161,0.5805,0.9289); rgb(84pt)=(0.1573,0.5854,0.9254); rgb(85pt)=(0.154,0.5902,0.9218); rgb(86pt)=(0.1513,0.595,0.9182); rgb(87pt)=(0.1492,0.5997,0.9147); rgb(88pt)=(0.1475,0.6043,0.9113); rgb(89pt)=(0.1461,0.6089,0.908); rgb(90pt)=(0.1446,0.6135,0.905); rgb(91pt)=(0.1429,0.618,0.9022); rgb(92pt)=(0.1408,0.6226,0.8998); rgb(93pt)=(0.1383,0.6272,0.8975); rgb(94pt)=(0.1354,0.6317,0.8953); rgb(95pt)=(0.1321,0.6363,0.8932); rgb(96pt)=(0.1288,0.6408,0.891); rgb(97pt)=(0.1253,0.6453,0.8887); rgb(98pt)=(0.1219,0.6497,0.8862); rgb(99pt)=(0.1185,0.6541,0.8834); rgb(100pt)=(0.1152,0.6584,0.8804); rgb(101pt)=(0.1119,0.6627,0.877); rgb(102pt)=(0.1085,0.6669,0.8734); rgb(103pt)=(0.1048,0.671,0.8695); rgb(104pt)=(0.1009,0.675,0.8653); rgb(105pt)=(0.0964,0.6789,0.8609); rgb(106pt)=(0.0914,0.6828,0.8562); rgb(107pt)=(0.0855,0.6865,0.8513); rgb(108pt)=(0.0789,0.6902,0.8462); rgb(109pt)=(0.0713,0.6938,0.8409); rgb(110pt)=(0.0628,0.6972,0.8355); rgb(111pt)=(0.0535,0.7006,0.8299); rgb(112pt)=(0.0433,0.7039,0.8242); rgb(113pt)=(0.0328,0.7071,0.8183); rgb(114pt)=(0.0234,0.7103,0.8124); rgb(115pt)=(0.0155,0.7133,0.8064); rgb(116pt)=(0.0091,0.7163,0.8003); rgb(117pt)=(0.0046,0.7192,0.7941); rgb(118pt)=(0.0019,0.722,0.7878); rgb(119pt)=(0.0009,0.7248,0.7815); rgb(120pt)=(0.0018,0.7275,0.7752); rgb(121pt)=(0.0046,0.7301,0.7688); rgb(122pt)=(0.0094,0.7327,0.7623); rgb(123pt)=(0.0162,0.7352,0.7558); rgb(124pt)=(0.0253,0.7376,0.7492); rgb(125pt)=(0.0369,0.74,0.7426); rgb(126pt)=(0.0504,0.7423,0.7359); rgb(127pt)=(0.0638,0.7446,0.7292); rgb(128pt)=(0.077,0.7468,0.7224); rgb(129pt)=(0.0899,0.7489,0.7156); rgb(130pt)=(0.1023,0.751,0.7088); rgb(131pt)=(0.1141,0.7531,0.7019); rgb(132pt)=(0.1252,0.7552,0.695); rgb(133pt)=(0.1354,0.7572,0.6881); rgb(134pt)=(0.1448,0.7593,0.6812); rgb(135pt)=(0.1532,0.7614,0.6741); rgb(136pt)=(0.1609,0.7635,0.6671); rgb(137pt)=(0.1678,0.7656,0.6599); rgb(138pt)=(0.1741,0.7678,0.6527); rgb(139pt)=(0.1799,0.7699,0.6454); rgb(140pt)=(0.1853,0.7721,0.6379); rgb(141pt)=(0.1905,0.7743,0.6303); rgb(142pt)=(0.1954,0.7765,0.6225); rgb(143pt)=(0.2003,0.7787,0.6146); rgb(144pt)=(0.2061,0.7808,0.6065); rgb(145pt)=(0.2118,0.7828,0.5983); rgb(146pt)=(0.2178,0.7849,0.5899); rgb(147pt)=(0.2244,0.7869,0.5813); rgb(148pt)=(0.2318,0.7887,0.5725); rgb(149pt)=(0.2401,0.7905,0.5636); rgb(150pt)=(0.2491,0.7922,0.5546); rgb(151pt)=(0.2589,0.7937,0.5454); rgb(152pt)=(0.2695,0.7951,0.536); rgb(153pt)=(0.2809,0.7964,0.5266); rgb(154pt)=(0.2929,0.7975,0.517); rgb(155pt)=(0.3052,0.7985,0.5074); rgb(156pt)=(0.3176,0.7994,0.4975); rgb(157pt)=(0.3301,0.8002,0.4876); rgb(158pt)=(0.3424,0.8009,0.4774); rgb(159pt)=(0.3548,0.8016,0.4669); rgb(160pt)=(0.3671,0.8021,0.4563); rgb(161pt)=(0.3795,0.8026,0.4454); rgb(162pt)=(0.3921,0.8029,0.4344); rgb(163pt)=(0.405,0.8031,0.4233); rgb(164pt)=(0.4184,0.803,0.4122); rgb(165pt)=(0.4322,0.8028,0.4013); rgb(166pt)=(0.4463,0.8024,0.3904); rgb(167pt)=(0.4608,0.8018,0.3797); rgb(168pt)=(0.4753,0.8011,0.3691); rgb(169pt)=(0.4899,0.8002,0.3586); rgb(170pt)=(0.5044,0.7993,0.348); rgb(171pt)=(0.5187,0.7982,0.3374); rgb(172pt)=(0.5329,0.797,0.3267); rgb(173pt)=(0.547,0.7957,0.3159); rgb(175pt)=(0.5748,0.7929,0.2941); rgb(176pt)=(0.5886,0.7913,0.2833); rgb(177pt)=(0.6024,0.7896,0.2726); rgb(178pt)=(0.6161,0.7878,0.2622); rgb(179pt)=(0.6297,0.7859,0.2521); rgb(180pt)=(0.6433,0.7839,0.2423); rgb(181pt)=(0.6567,0.7818,0.2329); rgb(182pt)=(0.6701,0.7796,0.2239); rgb(183pt)=(0.6833,0.7773,0.2155); rgb(184pt)=(0.6963,0.775,0.2075); rgb(185pt)=(0.7091,0.7727,0.1998); rgb(186pt)=(0.7218,0.7703,0.1924); rgb(187pt)=(0.7344,0.7679,0.1852); rgb(188pt)=(0.7468,0.7654,0.1782); rgb(189pt)=(0.759,0.7629,0.1717); rgb(190pt)=(0.771,0.7604,0.1658); rgb(191pt)=(0.7829,0.7579,0.1608); rgb(192pt)=(0.7945,0.7554,0.157); rgb(193pt)=(0.806,0.7529,0.1546); rgb(194pt)=(0.8172,0.7505,0.1535); rgb(195pt)=(0.8281,0.7481,0.1536); rgb(196pt)=(0.8389,0.7457,0.1546); rgb(197pt)=(0.8495,0.7435,0.1564); rgb(198pt)=(0.86,0.7413,0.1587); rgb(199pt)=(0.8703,0.7392,0.1615); rgb(200pt)=(0.8804,0.7372,0.165); rgb(201pt)=(0.8903,0.7353,0.1695); rgb(202pt)=(0.9,0.7336,0.1749); rgb(203pt)=(0.9093,0.7321,0.1815); rgb(204pt)=(0.9184,0.7308,0.189); rgb(205pt)=(0.9272,0.7298,0.1973); rgb(206pt)=(0.9357,0.729,0.2061); rgb(207pt)=(0.944,0.7285,0.2151); rgb(208pt)=(0.9523,0.7284,0.2237); rgb(209pt)=(0.9606,0.7285,0.2312); rgb(210pt)=(0.9689,0.7292,0.2373); rgb(211pt)=(0.977,0.7304,0.2418); rgb(212pt)=(0.9842,0.733,0.2446); rgb(213pt)=(0.99,0.7365,0.2429); rgb(214pt)=(0.9946,0.7407,0.2394); rgb(215pt)=(0.9966,0.7458,0.2351); rgb(216pt)=(0.9971,0.7513,0.2309); rgb(217pt)=(0.9972,0.7569,0.2267); rgb(218pt)=(0.9971,0.7626,0.2224); rgb(219pt)=(0.9969,0.7683,0.2181); rgb(220pt)=(0.9966,0.774,0.2138); rgb(221pt)=(0.9962,0.7798,0.2095); rgb(222pt)=(0.9957,0.7856,0.2053); rgb(223pt)=(0.9949,0.7915,0.2012); rgb(224pt)=(0.9938,0.7974,0.1974); rgb(225pt)=(0.9923,0.8034,0.1939); rgb(226pt)=(0.9906,0.8095,0.1906); rgb(227pt)=(0.9885,0.8156,0.1875); rgb(228pt)=(0.9861,0.8218,0.1846); rgb(229pt)=(0.9835,0.828,0.1817); rgb(230pt)=(0.9807,0.8342,0.1787); rgb(231pt)=(0.9778,0.8404,0.1757); rgb(232pt)=(0.9748,0.8467,0.1726); rgb(233pt)=(0.972,0.8529,0.1695); rgb(234pt)=(0.9694,0.8591,0.1665); rgb(235pt)=(0.9671,0.8654,0.1636); rgb(236pt)=(0.9651,0.8716,0.1608); rgb(237pt)=(0.9634,0.8778,0.1582); rgb(238pt)=(0.9619,0.884,0.1557); rgb(239pt)=(0.9608,0.8902,0.1532); rgb(240pt)=(0.9601,0.8963,0.1507); rgb(241pt)=(0.9596,0.9023,0.148); rgb(242pt)=(0.9595,0.9084,0.145); rgb(243pt)=(0.9597,0.9143,0.1418); rgb(244pt)=(0.9601,0.9203,0.1382); rgb(245pt)=(0.9608,0.9262,0.1344); rgb(246pt)=(0.9618,0.932,0.1304); rgb(247pt)=(0.9629,0.9379,0.1261); rgb(248pt)=(0.9642,0.9437,0.1216); rgb(249pt)=(0.9657,0.9494,0.1168); rgb(250pt)=(0.9674,0.9552,0.1116); rgb(251pt)=(0.9692,0.9609,0.1061); rgb(252pt)=(0.9711,0.9667,0.1001); rgb(253pt)=(0.973,0.9724,0.0938); rgb(254pt)=(0.9749,0.9782,0.0872); rgb(255pt)=(0.9769,0.9839,0.0805)}, mesh/rows=101]
table[point meta=\thisrow{c}] {%
\datapath/cost_coherent_20_dB_pos-1.tsv};
\addlegendentry{ML Cost Function}

\addplot3 [color=black, dashed, line width=2.0pt]
 table[] {\datapath/cost_coherent_20_dB_pos-2.tsv};
 \addlegendentry{Ground-Truth}

\addplot3 [color=mycolor1, dashdotted, line width=2.0pt]
 table[] {\datapath/cost_coherent_20_dB_pos-3.tsv};
 \addlegendentry{Estimate}

\end{axis}
\end{tikzpicture}%

==> Figures/Estimator_figures/cost_noncoherent_20_dB_pos/cost_noncoherent_20_dB_pos.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=2.3735,
xmax=3.4,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={Y-Coordinate [m]},
ymin=2.5,
ymax=3.5297,
ylabel style={font=\color{white!15!black}},
ylabel={X-Coordinate [m]},
zmin=-9.28376347392758,
zmax=0,
zlabel style={font=\color{white!15!black}},
zlabel={ML Cost Function [dB]},
view={45}{19},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
zmajorgrids,
legend style={at={(0.553,0.789)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]

\addplot3[%
surf,
shader=flat corner, fill=white, z buffer=sort, colormap={mymap}{[1pt] rgb(0pt)=(0.2422,0.1504,0.6603); rgb(1pt)=(0.2444,0.1534,0.6728); rgb(2pt)=(0.2464,0.1569,0.6847); rgb(3pt)=(0.2484,0.1607,0.6961); rgb(4pt)=(0.2503,0.1648,0.7071); rgb(5pt)=(0.2522,0.1689,0.7179); rgb(6pt)=(0.254,0.1732,0.7286); rgb(7pt)=(0.2558,0.1773,0.7393); rgb(8pt)=(0.2576,0.1814,0.7501); rgb(9pt)=(0.2594,0.1854,0.761); rgb(11pt)=(0.2628,0.1932,0.7828); rgb(12pt)=(0.2645,0.1972,0.7937); rgb(13pt)=(0.2661,0.2011,0.8043); rgb(14pt)=(0.2676,0.2052,0.8148); rgb(15pt)=(0.2691,0.2094,0.8249); rgb(16pt)=(0.2704,0.2138,0.8346); rgb(17pt)=(0.2717,0.2184,0.8439); rgb(18pt)=(0.2729,0.2231,0.8528); rgb(19pt)=(0.274,0.228,0.8612); rgb(20pt)=(0.2749,0.233,0.8692); rgb(21pt)=(0.2758,0.2382,0.8767); rgb(22pt)=(0.2766,0.2435,0.884); rgb(23pt)=(0.2774,0.2489,0.8908); rgb(24pt)=(0.2781,0.2543,0.8973); rgb(25pt)=(0.2788,0.2598,0.9035); rgb(26pt)=(0.2794,0.2653,0.9094); rgb(27pt)=(0.2798,0.2708,0.915); rgb(28pt)=(0.2802,0.2764,0.9204); rgb(29pt)=(0.2806,0.2819,0.9255); rgb(30pt)=(0.2809,0.2875,0.9305); rgb(31pt)=(0.2811,0.293,0.9352); rgb(32pt)=(0.2813,0.2985,0.9397); rgb(33pt)=(0.2814,0.304,0.9441); rgb(34pt)=(0.2814,0.3095,0.9483); rgb(35pt)=(0.2813,0.315,0.9524); rgb(36pt)=(0.2811,0.3204,0.9563); rgb(37pt)=(0.2809,0.3259,0.96); rgb(38pt)=(0.2807,0.3313,0.9636); rgb(39pt)=(0.2803,0.3367,0.967); rgb(40pt)=(0.2798,0.3421,0.9702); rgb(41pt)=(0.2791,0.3475,0.9733); rgb(42pt)=(0.2784,0.3529,0.9763); rgb(43pt)=(0.2776,0.3583,0.9791); rgb(44pt)=(0.2766,0.3638,0.9817); rgb(45pt)=(0.2754,0.3693,0.984); rgb(46pt)=(0.2741,0.3748,0.9862); rgb(47pt)=(0.2726,0.3804,0.9881); rgb(48pt)=(0.271,0.386,0.9898); rgb(49pt)=(0.2691,0.3916,0.9912); rgb(50pt)=(0.267,0.3973,0.9924); rgb(51pt)=(0.2647,0.403,0.9935); rgb(52pt)=(0.2621,0.4088,0.9946); rgb(53pt)=(0.2591,0.4145,0.9955); rgb(54pt)=(0.2556,0.4203,0.9965); rgb(55pt)=(0.2517,0.4261,0.9974); rgb(56pt)=(0.2473,0.4319,0.9983); rgb(57pt)=(0.2424,0.4378,0.9991); rgb(58pt)=(0.2369,0.4437,0.9996); rgb(59pt)=(0.2311,0.4497,0.9995); rgb(60pt)=(0.225,0.4559,0.9985); rgb(61pt)=(0.2189,0.462,0.9968); rgb(62pt)=(0.2128,0.4682,0.9948); rgb(63pt)=(0.2066,0.4743,0.9926); rgb(64pt)=(0.2006,0.4803,0.9906); rgb(65pt)=(0.195,0.4861,0.9887); rgb(66pt)=(0.1903,0.4919,0.9867); rgb(67pt)=(0.1869,0.4975,0.9844); rgb(68pt)=(0.1847,0.503,0.9819); rgb(69pt)=(0.1831,0.5084,0.9793); rgb(70pt)=(0.1818,0.5138,0.9766); rgb(71pt)=(0.1806,0.5191,0.9738); rgb(72pt)=(0.1795,0.5244,0.9709); rgb(73pt)=(0.1785,0.5296,0.9677); rgb(74pt)=(0.1778,0.5349,0.9641); rgb(75pt)=(0.1773,0.5401,0.9602); rgb(76pt)=(0.1768,0.5452,0.956); rgb(77pt)=(0.1764,0.5504,0.9516); rgb(78pt)=(0.1755,0.5554,0.9473); rgb(79pt)=(0.174,0.5605,0.9432); rgb(80pt)=(0.1716,0.5655,0.9393); rgb(81pt)=(0.1686,0.5705,0.9357); rgb(82pt)=(0.1649,0.5755,0.9323); rgb(83pt)=(0.161,0.5805,0.9289); rgb(84pt)=(0.1573,0.5854,0.9254); rgb(85pt)=(0.154,0.5902,0.9218); rgb(86pt)=(0.1513,0.595,0.9182); rgb(87pt)=(0.1492,0.5997,0.9147); rgb(88pt)=(0.1475,0.6043,0.9113); rgb(89pt)=(0.1461,0.6089,0.908); rgb(90pt)=(0.1446,0.6135,0.905); rgb(91pt)=(0.1429,0.618,0.9022); rgb(92pt)=(0.1408,0.6226,0.8998); rgb(93pt)=(0.1383,0.6272,0.8975); rgb(94pt)=(0.1354,0.6317,0.8953); rgb(95pt)=(0.1321,0.6363,0.8932); rgb(96pt)=(0.1288,0.6408,0.891); rgb(97pt)=(0.1253,0.6453,0.8887); rgb(98pt)=(0.1219,0.6497,0.8862); rgb(99pt)=(0.1185,0.6541,0.8834); rgb(100pt)=(0.1152,0.6584,0.8804); rgb(101pt)=(0.1119,0.6627,0.877); rgb(102pt)=(0.1085,0.6669,0.8734); rgb(103pt)=(0.1048,0.671,0.8695); rgb(104pt)=(0.1009,0.675,0.8653); rgb(105pt)=(0.0964,0.6789,0.8609); rgb(106pt)=(0.0914,0.6828,0.8562); rgb(107pt)=(0.0855,0.6865,0.8513); rgb(108pt)=(0.0789,0.6902,0.8462); rgb(109pt)=(0.0713,0.6938,0.8409); rgb(110pt)=(0.0628,0.6972,0.8355); rgb(111pt)=(0.0535,0.7006,0.8299); rgb(112pt)=(0.0433,0.7039,0.8242); rgb(113pt)=(0.0328,0.7071,0.8183); rgb(114pt)=(0.0234,0.7103,0.8124); rgb(115pt)=(0.0155,0.7133,0.8064); rgb(116pt)=(0.0091,0.7163,0.8003); rgb(117pt)=(0.0046,0.7192,0.7941); rgb(118pt)=(0.0019,0.722,0.7878); rgb(119pt)=(0.0009,0.7248,0.7815); rgb(120pt)=(0.0018,0.7275,0.7752); rgb(121pt)=(0.0046,0.7301,0.7688); rgb(122pt)=(0.0094,0.7327,0.7623); rgb(123pt)=(0.0162,0.7352,0.7558); rgb(124pt)=(0.0253,0.7376,0.7492); rgb(125pt)=(0.0369,0.74,0.7426); rgb(126pt)=(0.0504,0.7423,0.7359); rgb(127pt)=(0.0638,0.7446,0.7292); rgb(128pt)=(0.077,0.7468,0.7224); rgb(129pt)=(0.0899,0.7489,0.7156); rgb(130pt)=(0.1023,0.751,0.7088); rgb(131pt)=(0.1141,0.7531,0.7019); rgb(132pt)=(0.1252,0.7552,0.695); rgb(133pt)=(0.1354,0.7572,0.6881); rgb(134pt)=(0.1448,0.7593,0.6812); rgb(135pt)=(0.1532,0.7614,0.6741); rgb(136pt)=(0.1609,0.7635,0.6671); rgb(137pt)=(0.1678,0.7656,0.6599); rgb(138pt)=(0.1741,0.7678,0.6527); rgb(139pt)=(0.1799,0.7699,0.6454); rgb(140pt)=(0.1853,0.7721,0.6379); rgb(141pt)=(0.1905,0.7743,0.6303); rgb(142pt)=(0.1954,0.7765,0.6225); rgb(143pt)=(0.2003,0.7787,0.6146); rgb(144pt)=(0.2061,0.7808,0.6065); rgb(145pt)=(0.2118,0.7828,0.5983); rgb(146pt)=(0.2178,0.7849,0.5899); rgb(147pt)=(0.2244,0.7869,0.5813); rgb(148pt)=(0.2318,0.7887,0.5725); rgb(149pt)=(0.2401,0.7905,0.5636); rgb(150pt)=(0.2491,0.7922,0.5546); rgb(151pt)=(0.2589,0.7937,0.5454); rgb(152pt)=(0.2695,0.7951,0.536); rgb(153pt)=(0.2809,0.7964,0.5266); rgb(154pt)=(0.2929,0.7975,0.517); rgb(155pt)=(0.3052,0.7985,0.5074); rgb(156pt)=(0.3176,0.7994,0.4975); rgb(157pt)=(0.3301,0.8002,0.4876); rgb(158pt)=(0.3424,0.8009,0.4774); rgb(159pt)=(0.3548,0.8016,0.4669); rgb(160pt)=(0.3671,0.8021,0.4563); rgb(161pt)=(0.3795,0.8026,0.4454); rgb(162pt)=(0.3921,0.8029,0.4344); rgb(163pt)=(0.405,0.8031,0.4233); rgb(164pt)=(0.4184,0.803,0.4122); rgb(165pt)=(0.4322,0.8028,0.4013); rgb(166pt)=(0.4463,0.8024,0.3904); rgb(167pt)=(0.4608,0.8018,0.3797); rgb(168pt)=(0.4753,0.8011,0.3691); rgb(169pt)=(0.4899,0.8002,0.3586); rgb(170pt)=(0.5044,0.7993,0.348); rgb(171pt)=(0.5187,0.7982,0.3374); rgb(172pt)=(0.5329,0.797,0.3267); rgb(173pt)=(0.547,0.7957,0.3159); rgb(175pt)=(0.5748,0.7929,0.2941); rgb(176pt)=(0.5886,0.7913,0.2833); rgb(177pt)=(0.6024,0.7896,0.2726); rgb(178pt)=(0.6161,0.7878,0.2622); rgb(179pt)=(0.6297,0.7859,0.2521); rgb(180pt)=(0.6433,0.7839,0.2423); rgb(181pt)=(0.6567,0.7818,0.2329); rgb(182pt)=(0.6701,0.7796,0.2239); rgb(183pt)=(0.6833,0.7773,0.2155); rgb(184pt)=(0.6963,0.775,0.2075); rgb(185pt)=(0.7091,0.7727,0.1998); rgb(186pt)=(0.7218,0.7703,0.1924); rgb(187pt)=(0.7344,0.7679,0.1852); rgb(188pt)=(0.7468,0.7654,0.1782); rgb(189pt)=(0.759,0.7629,0.1717); rgb(190pt)=(0.771,0.7604,0.1658); rgb(191pt)=(0.7829,0.7579,0.1608); rgb(192pt)=(0.7945,0.7554,0.157); rgb(193pt)=(0.806,0.7529,0.1546); rgb(194pt)=(0.8172,0.7505,0.1535); rgb(195pt)=(0.8281,0.7481,0.1536); rgb(196pt)=(0.8389,0.7457,0.1546); rgb(197pt)=(0.8495,0.7435,0.1564); rgb(198pt)=(0.86,0.7413,0.1587); rgb(199pt)=(0.8703,0.7392,0.1615); rgb(200pt)=(0.8804,0.7372,0.165); rgb(201pt)=(0.8903,0.7353,0.1695); rgb(202pt)=(0.9,0.7336,0.1749); rgb(203pt)=(0.9093,0.7321,0.1815); rgb(204pt)=(0.9184,0.7308,0.189); rgb(205pt)=(0.9272,0.7298,0.1973); rgb(206pt)=(0.9357,0.729,0.2061); rgb(207pt)=(0.944,0.7285,0.2151); rgb(208pt)=(0.9523,0.7284,0.2237); rgb(209pt)=(0.9606,0.7285,0.2312); rgb(210pt)=(0.9689,0.7292,0.2373); rgb(211pt)=(0.977,0.7304,0.2418); rgb(212pt)=(0.9842,0.733,0.2446); rgb(213pt)=(0.99,0.7365,0.2429); rgb(214pt)=(0.9946,0.7407,0.2394); rgb(215pt)=(0.9966,0.7458,0.2351); rgb(216pt)=(0.9971,0.7513,0.2309); rgb(217pt)=(0.9972,0.7569,0.2267); rgb(218pt)=(0.9971,0.7626,0.2224); rgb(219pt)=(0.9969,0.7683,0.2181); rgb(220pt)=(0.9966,0.774,0.2138); rgb(221pt)=(0.9962,0.7798,0.2095); rgb(222pt)=(0.9957,0.7856,0.2053); rgb(223pt)=(0.9949,0.7915,0.2012); rgb(224pt)=(0.9938,0.7974,0.1974); rgb(225pt)=(0.9923,0.8034,0.1939); rgb(226pt)=(0.9906,0.8095,0.1906); rgb(227pt)=(0.9885,0.8156,0.1875); rgb(228pt)=(0.9861,0.8218,0.1846); rgb(229pt)=(0.9835,0.828,0.1817); rgb(230pt)=(0.9807,0.8342,0.1787); rgb(231pt)=(0.9778,0.8404,0.1757); rgb(232pt)=(0.9748,0.8467,0.1726); rgb(233pt)=(0.972,0.8529,0.1695); rgb(234pt)=(0.9694,0.8591,0.1665); rgb(235pt)=(0.9671,0.8654,0.1636); rgb(236pt)=(0.9651,0.8716,0.1608); rgb(237pt)=(0.9634,0.8778,0.1582); rgb(238pt)=(0.9619,0.884,0.1557); rgb(239pt)=(0.9608,0.8902,0.1532); rgb(240pt)=(0.9601,0.8963,0.1507); rgb(241pt)=(0.9596,0.9023,0.148); rgb(242pt)=(0.9595,0.9084,0.145); rgb(243pt)=(0.9597,0.9143,0.1418); rgb(244pt)=(0.9601,0.9203,0.1382); rgb(245pt)=(0.9608,0.9262,0.1344); rgb(246pt)=(0.9618,0.932,0.1304); rgb(247pt)=(0.9629,0.9379,0.1261); rgb(248pt)=(0.9642,0.9437,0.1216); rgb(249pt)=(0.9657,0.9494,0.1168); rgb(250pt)=(0.9674,0.9552,0.1116); rgb(251pt)=(0.9692,0.9609,0.1061); rgb(252pt)=(0.9711,0.9667,0.1001); rgb(253pt)=(0.973,0.9724,0.0938); rgb(254pt)=(0.9749,0.9782,0.0872); rgb(255pt)=(0.9769,0.9839,0.0805)}, mesh/rows=101]
table[point meta=\thisrow{c}] {%
\datapath/cost_noncoherent_20_dB_pos-1.tsv};
\addlegendentry{ML Cost Function}

\addplot3 [color=black, dashed, line width=2.0pt]
 table[] {\datapath/cost_noncoherent_20_dB_pos-2.tsv};
 \addlegendentry{Ground-Truth}

\addplot3 [color=mycolor1, dashdotted, line width=2.0pt]
 table[] {\datapath/cost_noncoherent_20_dB_pos-3.tsv};
 \addlegendentry{Estimate}

\end{axis}
\end{tikzpicture}%

==> Figures/Estimator_figures/cost_noncoherent_20_dB_pos_img/cost_noncoherent_20_dB_pos_img_CM.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\scriptsize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
% \colorlet{mycolor1}{white}

\begin{tikzpicture}[baseline,trim axis left]

\begin{axis}[%
width=0.855\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-8.4397849762978,
point meta max=0,
axis on top,
xmin=2.5247,
xmax=3.5347,
% xlabel style={font=\color{white!15!black}},
xlabel={$y$-coordinate in \SI{}{\metre}},
ymin=2.3685,
ymax=3.3785,
% ylabel style={font=\color{white!15!black}},
ylabel={$x$-coordinate in \SI{}{\metre}},
% axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={at={(1,1)},anchor=north east,legend cell align=left, align=left, draw=white!15!black,fill opacity=0.7,text opacity=1}, % nice
%extraAxisOptions,
% unit vector ratio=1 1 1,
colorbar horizontal,
colorbar style={at={(0,1.025)},anchor=south west,major tick length=1mm,height=1.75mm,xlabel=ML cost function in dB, yticklabel style={rotate=90,font=\footnotesize,xshift=-0.5mm}, ylabel style={yshift=1.5mm},ytick distance={30},xticklabel pos=upper},
colormap={mymap}{[1pt] rgb(0pt)=(0.995023,0.995023,0.995023); rgb(1pt)=(0.987523,0.989196,0.995075); rgb(2pt)=(0.980022,0.983369,0.995127); rgb(3pt)=(0.972521,0.977542,0.995179); rgb(4pt)=(0.96502,0.971714,0.995231); rgb(5pt)=(0.957519,0.965887,0.995283); rgb(6pt)=(0.950018,0.96006,0.995334); rgb(7pt)=(0.942517,0.954233,0.995386); rgb(8pt)=(0.935016,0.948405,0.995438); rgb(9pt)=(0.927515,0.942578,0.99549); rgb(10pt)=(0.920014,0.936751,0.995542); rgb(11pt)=(0.912513,0.930924,0.995594); rgb(12pt)=(0.905012,0.925096,0.995646); rgb(13pt)=(0.897512,0.919269,0.995697); rgb(14pt)=(0.890011,0.913442,0.995749); rgb(15pt)=(0.88251,0.907615,0.995801); rgb(16pt)=(0.875009,0.901787,0.995853); rgb(17pt)=(0.867508,0.89596,0.995905); rgb(18pt)=(0.860007,0.890133,0.995957); rgb(19pt)=(0.852506,0.884306,0.996008); rgb(20pt)=(0.845005,0.878478,0.99606); rgb(21pt)=(0.837504,0.872651,0.996112); rgb(22pt)=(0.830003,0.866824,0.996164); rgb(23pt)=(0.822502,0.860997,0.996216); rgb(24pt)=(0.815001,0.855169,0.996268); rgb(25pt)=(0.807501,0.849342,0.996319); rgb(26pt)=(0.8,0.843515,0.996371); rgb(27pt)=(0.792499,0.837687,0.996423); rgb(28pt)=(0.784998,0.83186,0.996475); rgb(29pt)=(0.777497,0.826033,0.996527); rgb(30pt)=(0.769996,0.820206,0.996579); rgb(31pt)=(0.762495,0.814378,0.99663); rgb(32pt)=(0.754994,0.808551,0.996682); rgb(33pt)=(0.747493,0.802724,0.996734); rgb(34pt)=(0.739992,0.796897,0.996786); rgb(35pt)=(0.732491,0.791069,0.996838); rgb(36pt)=(0.72499,0.785242,0.99689); rgb(37pt)=(0.71749,0.779415,0.996942); rgb(38pt)=(0.709989,0.773588,0.996993); rgb(39pt)=(0.702488,0.76776,0.997045); rgb(40pt)=(0.694987,0.761933,0.997097); rgb(41pt)=(0.687486,0.756106,0.997149); rgb(42pt)=(0.679985,0.750279,0.997201); rgb(43pt)=(0.672484,0.744451,0.997253); rgb(44pt)=(0.664983,0.738624,0.997304); rgb(45pt)=(0.657482,0.732797,0.997356); rgb(46pt)=(0.649981,0.72697,0.997408); rgb(48pt)=(0.634979,0.715315,0.997512); rgb(49pt)=(0.627479,0.709488,0.997564); rgb(50pt)=(0.619978,0.703661,0.997615); rgb(51pt)=(0.612477,0.697833,0.997667); rgb(52pt)=(0.604976,0.692006,0.997719); rgb(53pt)=(0.597475,0.686179,0.997771); rgb(54pt)=(0.589974,0.680352,0.997823); rgb(55pt)=(0.582473,0.674524,0.997875); rgb(56pt)=(0.574972,0.668697,0.997926); rgb(57pt)=(0.567471,0.66287,0.997978); rgb(58pt)=(0.55997,0.657043,0.99803); rgb(59pt)=(0.552469,0.651215,0.998082); rgb(60pt)=(0.544968,0.645388,0.998134); rgb(61pt)=(0.537468,0.639561,0.998186); rgb(62pt)=(0.529967,0.633734,0.998237); rgb(63pt)=(0.522466,0.627906,0.998289); rgb(64pt)=(0.514965,0.622079,0.998341); rgb(65pt)=(0.507464,0.616252,0.998393); rgb(66pt)=(0.499963,0.610424,0.998445); rgb(69pt)=(0.47746,0.592943,0.9986); rgb(70pt)=(0.469959,0.587115,0.998652); rgb(71pt)=(0.462458,0.581288,0.998704); rgb(72pt)=(0.454957,0.575461,0.998756); rgb(73pt)=(0.447457,0.569634,0.998808); rgb(76pt)=(0.424954,0.552152,0.998963); rgb(77pt)=(0.417453,0.546325,0.999015); rgb(79pt)=(0.402451,0.53467,0.999119); rgb(80pt)=(0.39495,0.528843,0.999171); rgb(82pt)=(0.379948,0.517188,0.999274); rgb(83pt)=(0.372447,0.511361,0.999326); rgb(84pt)=(0.364946,0.505534,0.999378); rgb(87pt)=(0.342444,0.488052,0.999533); rgb(88pt)=(0.334943,0.482225,0.999585); rgb(90pt)=(0.319941,0.47057,0.999689); rgb(91pt)=(0.31244,0.464743,0.999741); rgb(92pt)=(0.304939,0.458916,0.999793); rgb(94pt)=(0.289937,0.447261,0.999896); rgb(95pt)=(0.282436,0.441434,0.999948); rgb(96pt)=(0.274935,0.435607,1); rgb(97pt)=(0.287287,0.428177,0.982837); rgb(98pt)=(0.299638,0.420747,0.965675); rgb(99pt)=(0.311989,0.413317,0.948512); rgb(100pt)=(0.324341,0.405887,0.93135); rgb(101pt)=(0.336692,0.398458,0.914187); rgb(102pt)=(0.349043,0.391028,0.897024); rgb(103pt)=(0.361394,0.383598,0.879862); rgb(104pt)=(0.373746,0.376168,0.862699); rgb(106pt)=(0.398448,0.361308,0.828374); rgb(107pt)=(0.4108,0.353879,0.811211); rgb(108pt)=(0.423151,0.346449,0.794049); rgb(109pt)=(0.435502,0.339019,0.776886); rgb(110pt)=(0.447853,0.331589,0.759723); rgb(111pt)=(0.460205,0.324159,0.742561); rgb(112pt)=(0.472556,0.31673,0.725398); rgb(113pt)=(0.484907,0.3093,0.708235); rgb(114pt)=(0.497258,0.30187,0.691073); rgb(115pt)=(0.50961,0.29444,0.67391); rgb(116pt)=(0.521961,0.28701,0.656748); rgb(117pt)=(0.534312,0.27958,0.639585); rgb(118pt)=(0.546664,0.272151,0.622422); rgb(119pt)=(0.559015,0.264721,0.60526); rgb(120pt)=(0.571366,0.257291,0.588097); rgb(121pt)=(0.583717,0.249861,0.570934); rgb(123pt)=(0.60842,0.235001,0.536609); rgb(124pt)=(0.620771,0.227572,0.519447); rgb(126pt)=(0.645474,0.212712,0.485121); rgb(127pt)=(0.657825,0.205282,0.467959); rgb(128pt)=(0.670176,0.197852,0.450796); rgb(136pt)=(0.768986,0.138414,0.313495); rgb(137pt)=(0.781338,0.130984,0.296332); rgb(138pt)=(0.793689,0.123554,0.27917); rgb(139pt)=(0.80604,0.116124,0.262007); rgb(140pt)=(0.818392,0.108694,0.244845); rgb(141pt)=(0.830743,0.101265,0.227682); rgb(143pt)=(0.855445,0.086405,0.193357); rgb(144pt)=(0.867797,0.0789751,0.176194); rgb(146pt)=(0.892499,0.0641155,0.141869); rgb(147pt)=(0.90485,0.0566857,0.124706); rgb(148pt)=(0.917202,0.0492559,0.107544); rgb(149pt)=(0.929553,0.041826,0.090381); rgb(150pt)=(0.941904,0.0343962,0.0732183); rgb(151pt)=(0.942988,0.0540008,0.0717241); rgb(152pt)=(0.944072,0.0736055,0.0702298); rgb(153pt)=(0.945156,0.0932101,0.0687356); rgb(154pt)=(0.94624,0.112815,0.0672413); rgb(156pt)=(0.948409,0.152024,0.0642528); rgb(157pt)=(0.949493,0.171629,0.0627586); rgb(158pt)=(0.950577,0.191233,0.0612643); rgb(159pt)=(0.951661,0.210838,0.0597701); rgb(161pt)=(0.953829,0.250047,0.0567816); rgb(162pt)=(0.954913,0.269652,0.0552873); rgb(163pt)=(0.955997,0.289256,0.0537931); rgb(164pt)=(0.957081,0.308861,0.0522988); rgb(165pt)=(0.958165,0.328466,0.0508046); rgb(166pt)=(0.959249,0.34807,0.0493103); rgb(168pt)=(0.961417,0.38728,0.0463218); rgb(169pt)=(0.962501,0.406884,0.0448276); rgb(170pt)=(0.963586,0.426489,0.0433333); rgb(171pt)=(0.96467,0.446094,0.041839); rgb(172pt)=(0.965754,0.465698,0.0403448); rgb(173pt)=(0.966838,0.485303,0.0388505); rgb(174pt)=(0.967922,0.504907,0.0373563); rgb(175pt)=(0.969006,0.524512,0.035862); rgb(176pt)=(0.97009,0.544117,0.0343678); rgb(178pt)=(0.972258,0.583326,0.0313793); rgb(179pt)=(0.973342,0.602931,0.029885); rgb(180pt)=(0.974426,0.622535,0.0283908); rgb(181pt)=(0.97551,0.64214,0.0268965); rgb(183pt)=(0.977678,0.681349,0.023908); rgb(184pt)=(0.978762,0.700954,0.0224138); rgb(185pt)=(0.979847,0.720559,0.0209195); rgb(186pt)=(0.980931,0.740163,0.0194253); rgb(187pt)=(0.982015,0.759768,0.017931); rgb(188pt)=(0.983099,0.779372,0.0164368); rgb(189pt)=(0.984183,0.798977,0.0149425); rgb(190pt)=(0.985267,0.818582,0.0134483); rgb(191pt)=(0.986351,0.838186,0.011954); rgb(192pt)=(0.987435,0.857791,0.0104598); rgb(193pt)=(0.988519,0.877396,0.00896551); rgb(195pt)=(0.990687,0.916605,0.00597701); rgb(196pt)=(0.991771,0.936209,0.00448275); rgb(197pt)=(0.992855,0.955814,0.0029885); rgb(198pt)=(0.993939,0.975419,0.00149425); rgb(199pt)=(0.995023,0.995023,0)},
colorbar
]
\addplot [forget plot] graphics [xmin=2.5247, xmax=3.5347, ymin=2.3685, ymax=3.3785] {\datapath/cost_noncoherent_20_dB_pos_img-1.png};

\addplot[only marks, mark=o, mark options={}, mark size=3.25000pt, draw=mycolor1,line width = 0.7pt] table[]{\datapath/cost_noncoherent_20_dB_pos_img-1.tsv};
\addlegendentry{Estimate}

\addplot[only marks, mark=x, mark options={}, mark size=3.25000pt, draw=mycolor2,line width = 0.7pt] table[]{\datapath/cost_noncoherent_20_dB_pos_img-2.tsv};
\addlegendentry{Ground-Truth}

\end{axis}
\end{tikzpicture}%




==> Figures/Estimator_figures/crb_c_nc/crb_c_nc.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=-10,
xmax=30,
xlabel style={font=\color{white!15!black}},
xlabel={SDNR in dB},
ymode=log,
ymin=0.0001,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={PEB in m},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=red, dashed, mark=square, mark options={solid, red}]
  table[]{\datapath/crb_c_nc-1.tsv};
\addlegendentry{PEB coh.}

\addplot [color=red, dotted]
  table[]{\datapath/crb_c_nc-2.tsv};
\addlegendentry{PEB n.-coh.}

\end{axis}
\end{tikzpicture}%

==> Figures/Estimator_figures/phase_offset_rmse_vs_snr_v2/phase_offset_rmse_vs_snr_v2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\scriptsize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.46667,0.67451,0.18824}%
%
\colorlet{mycolor1}{IEEEblue}
\colorlet{mycolor2}{IEEEdarkorange}
\colorlet{mycolor3}{IEEElightgreen}

\begin{tikzpicture}[baseline,trim axis left]%baseline,

\begin{axis}[%
width=\figurewidth,
height=0.969\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
tick align=inside,		       % [B] ticks oriented inside 
axis line style = thick,	   % [B] thick axis lines 
xmin=-10,
xmax=30,
% xlabel style={font=\color{white!15!black}},
xlabel={SDNR in \SI{}{\dB}},
ymode=log,
ymin=0.1,
ymax=100,
yminorticks=true,
% ylabel style={font=\color{white!15!black}},
ylabel={Phase offset RMSE in \SI{}{\degree} },
% axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
grid style=dotted,
legend style={at={(1,1)}, legend columns=2, anchor=north east, 
legend cell align=left, align=left, draw=white!15!black},
fill=white,line cap = round, fill opacity=0.8, text opacity = 1, draw opacity = 1
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=mycolor1, dashdotted, line width=\linewidthA, mark size=\marksizeA, mark=o, mark options={solid, mycolor1}]
  table[]{\datapath/phase_offset_rmse_vs_snr_v2-1.tsv};
\addlegendentry{RML}

\addplot [color=mycolor2, line width=\linewidthA, mark size=\marksizeA, mark=+, mark options={solid, mycolor2}]
  table[]{\datapath/phase_offset_rmse_vs_snr_v2-2.tsv};
\addlegendentry{JML}

\addplot [color=mycolor3, dashed, line width=\linewidthA]
  table[]{\datapath/phase_offset_rmse_vs_snr_v2-3.tsv};
\addlegendentry{CRB}

\end{axis}
\end{tikzpicture}%

==> Figures/RMSE_CEB.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\tiny},
  tick label style={font=\footnotesize},
  % xticklabel={
  %   % test if the x value is below zero
  %   \ifdim \tick pt < 0pt
  %     % if yes, calculate the absolute value
  %     \pgfmathparse{abs(\tick)}%
  %     % and print first a minus sign in a zero-width box, followed by the absolute value
  %     \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
  %  \else
  %    % if no, print as usual
  %     \pgfmathprintnumber{\tick}
  %  \fi
% }
}}

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85098,0.32549,0.09804}%
\definecolor{mycolor3}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor4}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\plotWidth,
height=\plotHeight,
at={(0\plotWidth,0\plotWidth)},
scale only axis,
xmin=0,
xmax=25,
% xlabel style={font=\color{white!15!black}},
xlabel={$\overline{\mathrm{SDNR}}$ in \unit{\dB}},
ymode=log,
ymin=0.1,
ymax=500,%1000,
yminorticks=true,
%ylabel style={font=\color{white!15!black}},
ylabel={RMSE in \unit{\nano\second}},%{\footnotesize RMSE [ns]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
xlabel style={yshift=0.2cm},
ylabel style={yshift=-0.2cm},
grid style=dotted,
legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black,legend columns=3}
% legend style={at={(0.749,0.6709)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black, font=\tiny}
]

\addplot [color=mycolor4, line width=1.25pt, mark size=2pt, mark=square, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0	98.8945967\\
5	56.5824915824916\\
10	12\\
15	1\\
20	0.254621319963631\\
25	0.123938411695197\\
};
\addlegendentry{ML}

\addplot [color=mycolor2, line width=1.25pt, mark size=2pt, mark=diamond, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0	126.666666666667\\
5	86.7849510705\\
10	32.974893898\\
15	11.5360382111434\\
20	3.24621319963631\\
25	1.62384116951966\\
};
\addlegendentry{ML-NCP}


\addplot [color=mycolor1, line width=1.25pt, mark size=2.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0	166.6667\\
5	126.4\\
10	78.1156\\
15	34.536\\
20	7.3462\\
25	3.2384\\
};
\addlegendentry{ILS}

% \addplot [color=red, dashed, line width=1.5pt]
\addplot [color=black, densely dashed, line width=1.5pt]
  table[row sep=crcr]{%
0	2.20327297345358\\
5	1.23899144364767\\
10	0.69673609032029\\
15	0.391803496338713\\
20	0.220327297345345\\
25	0.123899144364776\\
};
\addlegendentry{CEB}

% \addplot [color=mycolor3, dashed, line width=1.5pt]
\addplot [color=black, dashdotted, line width=1.5pt]
  table[row sep=crcr]{%
0	28.6365285666727\\
5	16.1035034242149\\
10	9.05566545659043\\
15	5.09237491382638\\
20	2.86365285696881\\
25	1.61035034284843\\
};
\addlegendentry{CEB-NCP}

\end{axis}

% \begin{axis}[%
% width=8.556in,
% height=5.875in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
% \end{axis}
\end{tikzpicture}%

==> Figures/RMSE_PEB.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\tiny},
  tick label style={font=\footnotesize},
  % xticklabel={
  %   % test if the x value is below zero
  %   \ifdim \tick pt < 0pt
  %     % if yes, calculate the absolute value
  %     \pgfmathparse{abs(\tick)}%
  %     % and print first a minus sign in a zero-width box, followed by the absolute value
  %     \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
  %  \else
  %    % if no, print as usual
  %     \pgfmathprintnumber{\tick}
  %  \fi
% }
}}

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85098,0.32549,0.09804}%
\definecolor{mycolor3}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor4}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=\plotWidth,
height=\plotHeight,
at={(0\plotWidth,0\plotWidth)},
scale only axis,
xmin=0,
xmax=25,
% xlabel style={font=\color{white!15!black}},
xlabel={$\overline{\mathrm{SDNR}}$ in \unit{\dB}},
ymode=log,
ymin=0.0007,%0.0005,%0.0001,
ymax=5,%9.99999999999999,
yminorticks=true,
% ylabel style={font=\color{white!15!black}},
ylabel={RMSE in \unit{\metre}},
xlabel style={yshift=0.2cm},
ylabel style={yshift=-0.2cm},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
grid style=dotted,
legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, fill=white, draw=white!15!black,legend columns=3}
%legend style={at={(1,1)}, anchor=north east, legend cell align=left, align=left, fill=white, fill opacity=0.6, draw opacity=1,text opacity=1, draw=white!15!black,font=\scriptsize,legend columns=3}
]

\addplot [color=mycolor4, line width=1.25pt, mark size=2pt, mark=square, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
0	2.82842712474619\\
5	1.58284271247462\\
10	0.372052057945166\\
15	0.011402051139295\\
20	0.001602284270196\\
25	0.000713947416988668\\
};
\addlegendentry{ML}

\addplot [color=mycolor2, line width=1.25pt, mark size=2pt, mark=diamond, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0	2.82842712474619\\
5	1.82842712474619\\
10	0.715562951706863\\
15	0.311853768147439\\
20	0.102356853057247\\
25	0.05320950246766\\
};
\addlegendentry{ML-NCP}

\addplot [color=mycolor1, line width=1.25pt, mark size=2.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0	3.28284271247462\\
5	2.285958\\
10	1.08174335110197\\
15	0.62925867293776\\
20	0.190901742920564\\
25	0.148698763819638\\
};
\addlegendentry{ILS}

% \addplot [color=red, dashed, line width=1.5pt]
\addplot [color=black, densely dashed, line width=1.5pt]
  table[row sep=crcr]{%
0	0.0125324086495412\\
5	0.00704749128780999\\
10	0.00396309559005451\\
15	0.00222861242596728\\
20	0.00125324086495412\\
25	0.000704749128781\\
};
\addlegendentry{PEB}

% \addplot [color=mycolor3, dashed, line width=1.5pt]
\addplot [color=black, dashdotted, line width=1.5pt]
  table[row sep=crcr]{%
0	0.939784263719636\\
5	0.528479528253195\\
10	0.297185878253664\\
15	0.167119900605051\\
20	0.0939784263718733\\
25	0.0528479528253056\\
};
\addlegendentry{PEB-NCP}

\end{axis}

% \begin{axis}[%
% width=8.556in,
% height=5.875in,
% at={(0in,0in)},
% scale only axis,
% xmin=0,
% xmax=1,
% ymin=0,
% ymax=1,
% axis line style={draw=none},
% ticks=none,
% axis x line*=bottom,
% axis y line*=left
% ]
% \end{axis}
\end{tikzpicture}%

==> Figures/bounds-sweep.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\tiny},
  tick label style={font=\footnotesize},
  % xticklabel={
  %   % test if the x value is below zero
  %   \ifdim \tick pt < 0pt
  %     % if yes, calculate the absolute value
  %     \pgfmathparse{abs(\tick)}%
  %     % and print first a minus sign in a zero-width box, followed by the absolute value
  %     \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
  %  \else
  %    % if no, print as usual
  %     \pgfmathprintnumber{\tick}
  %  \fi
% }
}}

\definecolor{NCP-M2}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{NCP-M4}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{NCP-M6}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{NCP-M8}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{CP-M2}{rgb}{0.00000,0.44700,0.74100}%{0.46600,0.67400,0.18800}%
\definecolor{CP-M4}{rgb}{0.85000,0.32500,0.09800}%{0.30100,0.74500,0.93300}%
\definecolor{CP-M6}{rgb}{0.92900,0.69400,0.12500}%{0.63500,0.07800,0.18400}%
\definecolor{CP-M8}{rgb}{0.49400,0.18400,0.55600}%{0.63500,0.07800,0.18400}%
%
\begin{tikzpicture}[spy using outlines={circle, magnification=2000, size=1cm, connect spies}]

\begin{axis}[%
width=\plotWidth,
height=\plotHeight,
at={(0\plotWidth,0\plotWidth)},
scale only axis,
xmode=log,
xmin=1000000,
xmax=1000000000,
xminorticks=true,
%xlabel style={font=\footnotesize},
xlabel={$B$ in \unit{\hertz}},
xlabel style={yshift=0.2cm},
ymode=log,
%ymin=0.002166,%0.001,
%ymax=0.002169,%1,
ymin=0.001,
ymax=1,
yminorticks=true,
%ylabel style={font=\footnotesize},
ylabel={$\peb$ in \unit{\metre}},
ylabel style={yshift=-0.2cm},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={avg. SDNR = 14.5dB},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
grid style=dotted,
%legend style={at={(1,1)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black,legend columns=2,font=\scriptsize}
legend style={at={(0.02,0.4)}, rotate=90, anchor=west, legend cell align=left, align=left, draw=white!15!black,legend columns=2}
]
\addplot [color=NCP-M2,mark=triangle,mark options={solid}, line width=1.25pt, line cap = round]
  table[row sep=crcr]{%
1000000	0.544344155853623\\
2000000	0.542877634045264\\
4000000	0.538797612710415\\
10000000	0.522574805367939\\
20000000	0.489333486803425\\
40000000	0.423610452635098\\
100000000	0.288645135681258\\
200000000	0.164622434077007\\
400000000	0.0681830227913661\\
1000000000	0.0265086734391372\\
};
\addlegendentry{NCP ($M=2$)}

\addplot [color=NCP-M4,mark=triangle,mark options={solid,rotate=90}, line width=1.25pt, line cap = round]
  table[row sep=crcr]{%
1000000	0.244172174334094\\
2000000	0.24403930669856\\
4000000	0.243664880448553\\
10000000	0.242103863446712\\
20000000	0.23850784003465\\
40000000	0.229447731113291\\
100000000	0.197919685044466\\
200000000	0.140562001407277\\
400000000	0.0660855692901826\\
1000000000	0.0263800732459715\\
};
\addlegendentry{NCP ($M=4$)}

\addplot [color=NCP-M6,mark=square,mark options={solid}, line width=1.25pt, line cap = round]
  table[row sep=crcr]{%
1000000	0.159917234594042\\
2000000	0.15987988752285\\
4000000	0.159774445326652\\
10000000	0.15933170448521\\
20000000	0.158292258365614\\
40000000	0.155548768077082\\
100000000	0.144469926838697\\
200000000	0.116871494952255\\
400000000	0.0629963854706102\\
1000000000	0.0261700206531866\\
};
\addlegendentry{NCP ($M=6$)}

\addplot [color=NCP-M8,mark=o,mark options={solid}, line width=1.25pt, line cap = round]
  table[row sep=crcr]{%
1000000	0.119212433899954\\
2000000	0.119196959438108\\
4000000	0.119153243022209\\
10000000	0.118969242055698\\
20000000	0.118534449737068\\
40000000	0.117367827608598\\
100000000	0.112367785828886\\
200000000	0.0977497099593659\\
400000000	0.0593376474750853\\
1000000000	0.0258845583837769\\
};
\addlegendentry{NCP ($M=8$)}

% \addplot [color=CP-M2, line width=0.001pt,forget plot]
%   table[row sep=crcr]{%
% 1000000	0.00216785190344958\\
% 2000000	0.00216754530947392\\
% 4000000	0.00216693230769148\\
% 10000000	0.0021650950736141\\
% 20000000	0.0021620391751095\\
% 40000000	0.0021559513493482\\
% 100000000	0.00213788095338152\\
% 200000000	0.00210836194274506\\
% 400000000	0.0020511580805722\\
% 1000000000	0.00189467065243163\\
% };
%\addlegendentry{Coherent}

% \addplot [color=CP-M4, line width=0.001pt, forget plot]
%   table[row sep=crcr]{%
% 1000000	0.00216778102157262\\
% 2000000	0.00216747445766563\\
% 4000000	0.0021668615159767\\
% 10000000	0.00216502446180276\\
% 20000000	0.00216196886185863\\
% 40000000	0.00215588162836581\\
% 100000000	0.00213781297081455\\
% 200000000	0.00210829673741194\\
% 400000000	0.00205109803981452\\
% 1000000000	0.00189462333153691\\
% };
% \addplot [color=CP-M6, line width=0.001pt, forget plot]
%   table[row sep=crcr]{%
% 1000000	0.00216766290128537\\
% 2000000	0.00216735638748135\\
% 4000000	0.00216674354592547\\
% 10000000	0.00216490679152225\\
% 20000000	0.00216185168906585\\
% 40000000	0.00215576544246377\\
% 100000000	0.0021376996816231\\
% 200000000	0.00210818807593048\\
% 400000000	0.00205099798415052\\
% 1000000000	0.00189454447162744\\
% };
% \addplot [color=CP-M8, line width=0.001pt, forget plot]
%   table[row sep=crcr]{%
% 1000000	0.00216749756683927\\
% 2000000	0.00216719112315539\\
% 4000000	0.00216657842173784\\
% 10000000	0.00216474208687027\\
% 20000000	0.00216168768065928\\
% 40000000	0.0021556028152353\\
% 100000000	0.00213754110842832\\
% 200000000	0.00210803597940298\\
% 400000000	0.00205085793197155\\
% 1000000000	0.00189443408507189\\
% };
%\spy [black] on (axis cs:3000000,0.0021678) in node at (4.5,1.7);
\addplot [densely dashed,mark=o,mark options={solid},color=black, line width=1.25pt, line cap = round]
  table[row sep=crcr]{%
1000000	0.00216749756683927\\
2000000	0.00216719112315539\\
4000000	0.00216657842173784\\
10000000	0.00216474208687027\\
20000000	0.00216168768065928\\
40000000	0.0021556028152353\\
100000000	0.00213754110842832\\
200000000	0.00210803597940298\\
400000000	0.00205085793197155\\
1000000000	0.00189443408507189\\
};
\addlegendentry{CP ($M=2\dots8$)}

% \addlegendimage{legend image with text=$ax$}
% \addlegendentry{}
\end{axis}
%\spy [black] on (0.15,0.4977) in node at (4.5,1.7);

%\draw (current bounding box.south west) rectangle (current bounding box.north east);
\end{tikzpicture}%

==> Figures/bounds-sweep_v2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{NCP-M2}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{NCP-M4}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{NCP-M6}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{NCP-M8}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{CP-M2}{rgb}{0.00000,0.44700,0.74100}%{0.46600,0.67400,0.18800}%
\definecolor{CP-M4}{rgb}{0.85000,0.32500,0.09800}%{0.30100,0.74500,0.93300}%
\definecolor{CP-M6}{rgb}{0.92900,0.69400,0.12500}%{0.63500,0.07800,0.18400}%
\definecolor{CP-M8}{rgb}{0.49400,0.18400,0.55600}%{0.63500,0.07800,0.18400}%
%
\def\yaxisscaling{1000}

\begin{tikzpicture}[spy using outlines={circle, magnification=100, size=1cm, connect spies}]

\begin{axis}[%
y filter/.code={\pgfmathparse{#1*\yaxisscaling}\pgfmathresult},
width=\plotWidth,
height=\plotHeight,
at={(0\plotWidth,0\plotWidth)},
scale only axis,
xmode=log,
xmin=1000000,
xmax=1000000000,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$B$ in Hz},
ymode=log,
%ymin=0.002166,%0.001,
%ymax=0.002169,%1,
ymin=0.006*\yaxisscaling,
ymax=0.01*\yaxisscaling,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\peb$ in m},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={avg. SDNR = 14.5dB},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.02,0.4)}, anchor=west, legend cell align=left, align=left, draw=white!15!black,font=\footnotesize}
]
% \addplot [color=NCP-M2, line width=1.5pt]
%   table[row sep=crcr]{%
% 1000000	0.544344155853623\\
% 2000000	0.542877634045264\\
% 4000000	0.538797612710415\\
% 10000000	0.522574805367939\\
% 20000000	0.489333486803425\\
% 40000000	0.423610452635098\\
% 100000000	0.288645135681258\\
% 200000000	0.164622434077007\\
% 400000000	0.0681830227913661\\
% 1000000000	0.0265086734391372\\
% };
% \addlegendentry{M=2}

% \addplot [color=NCP-M4, line width=1.5pt]
%   table[row sep=crcr]{%
% 1000000	0.244172174334094\\
% 2000000	0.24403930669856\\
% 4000000	0.243664880448553\\
% 10000000	0.242103863446712\\
% 20000000	0.23850784003465\\
% 40000000	0.229447731113291\\
% 100000000	0.197919685044466\\
% 200000000	0.140562001407277\\
% 400000000	0.0660855692901826\\
% 1000000000	0.0263800732459715\\
% };
% \addlegendentry{M=4}

% \addplot [color=NCP-M6, line width=1.5pt]
%   table[row sep=crcr]{%
% 1000000	0.159917234594042\\
% 2000000	0.15987988752285\\
% 4000000	0.159774445326652\\
% 10000000	0.15933170448521\\
% 20000000	0.158292258365614\\
% 40000000	0.155548768077082\\
% 100000000	0.144469926838697\\
% 200000000	0.116871494952255\\
% 400000000	0.0629963854706102\\
% 1000000000	0.0261700206531866\\
% };
% \addlegendentry{M=6}

% \addplot [color=NCP-M8, line width=1.5pt]
%   table[row sep=crcr]{%
% 1000000	0.119212433899954\\
% 2000000	0.119196959438108\\
% 4000000	0.119153243022209\\
% 10000000	0.118969242055698\\
% 20000000	0.118534449737068\\
% 40000000	0.117367827608598\\
% 100000000	0.112367785828886\\
% 200000000	0.0977497099593659\\
% 400000000	0.0593376474750853\\
% 1000000000	0.0258845583837769\\
% };
% \addlegendentry{M=8}

\addplot [color=CP-M2, line width=0.001pt,forget plot]
  table[row sep=crcr]{%
1000000	0.00216785190344958\\
2000000	0.00216754530947392\\
4000000	0.00216693230769148\\
10000000	0.0021650950736141\\
20000000	0.0021620391751095\\
40000000	0.0021559513493482\\
100000000	0.00213788095338152\\
200000000	0.00210836194274506\\
400000000	0.0020511580805722\\
1000000000	0.00189467065243163\\
};
%\addlegendentry{Coherent}

\addplot [color=CP-M4, line width=0.001pt, forget plot]
  table[row sep=crcr]{%
1000000	0.00216778102157262\\
2000000	0.00216747445766563\\
4000000	0.0021668615159767\\
10000000	0.00216502446180276\\
20000000	0.00216196886185863\\
40000000	0.00215588162836581\\
100000000	0.00213781297081455\\
200000000	0.00210829673741194\\
400000000	0.00205109803981452\\
1000000000	0.00189462333153691\\
};
\addplot [color=CP-M6, line width=0.001pt, forget plot]
  table[row sep=crcr]{%
1000000	0.00216766290128537\\
2000000	0.00216735638748135\\
4000000	0.00216674354592547\\
10000000	0.00216490679152225\\
20000000	0.00216185168906585\\
40000000	0.00215576544246377\\
100000000	0.0021376996816231\\
200000000	0.00210818807593048\\
400000000	0.00205099798415052\\
1000000000	0.00189454447162744\\
};
\addplot [color=CP-M8, line width=0.001pt, forget plot]
  table[row sep=crcr]{%
1000000	0.00216749756683927\\
2000000	0.00216719112315539\\
4000000	0.00216657842173784\\
10000000	0.00216474208687027\\
20000000	0.00216168768065928\\
40000000	0.0021556028152353\\
100000000	0.00213754110842832\\
200000000	0.00210803597940298\\
400000000	0.00205085793197155\\
1000000000	0.00189443408507189\\
};
%\spy [black] on (axis cs:3000000,0.0021678) in node at (4.5,1.7);
\addplot [dashed,color=black, line width=1.5pt]
  table[row sep=crcr]{%
1000000	0.00216749756683927\\
2000000	0.00216719112315539\\
4000000	0.00216657842173784\\
10000000	0.00216474208687027\\
20000000	0.00216168768065928\\
40000000	0.0021556028152353\\
100000000	0.00213754110842832\\
200000000	0.00210803597940298\\
400000000	0.00205085793197155\\
1000000000	0.00189443408507189\\
};
\addlegendentry{CP ($M=2,\dots,8$)}
\end{axis}
\spy [black] on (0.15,1.635) in node at (4.5,1.7);
\end{tikzpicture}%

==> Figures/externalized/foo.tex <==
% This file is needed on Overleaf to keep this folder for externalizing tikz figures.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}


==> shield-commands.tex <==
\ifx\SI\undefined
    \newcommand{\SI}[2]{{\color{red}SI-PKG-MISSING}}
    \newcommand{\giga}[0]{0}
    \newcommand{\hertz}[0]{0}
    \newcommand{\dB}[0]{0}
    \newcommand{\dBm}[0]{0}
    \newcommand{\num}[1]{0}
    \newcommand{\roundlabel}[1]{{\color{red}ROUND-LBL-MISSING}}
    \newcommand{\roundlabeltxt}[1]{{\color{red}ROUND-LBL-MISSING}}
    \newcommand{\missing}[0]{0}
\else
  %% Do this if it is defined
\fi
